Deep Reinforcement Agent for Efficient Instant Search

Instant Search is a paradigm where a search system retrieves answers on the fly while typing. The na\"ive implementation of an Instant Search system would hit the search back-end for results each time a user types a key, imposing a very high load on the underlying search system. In this paper, we propose to address the load issue by identifying tokens that are semantically more salient towards retrieving relevant documents and utilize this knowledge to trigger an instant search selectively. We train a reinforcement agent that interacts directly with the search engine and learns to predict the word's importance. Our proposed method treats the underlying search system as a black box and is more universally applicable to a diverse set of architectures. Furthermore, a novel evaluation framework is presented to study the trade-off between the number of triggered searches and the system's performance. We utilize the framework to evaluate and compare the proposed reinforcement method with other intuitive baselines. Experimental results demonstrate the efficacy of the proposed method towards achieving a superior trade-off.

==> analysis.tex <==

%While core metrics \acrshort{delay} and \acrshort{ts} are essential to measure the overall Load-Interactivity trade-off, they are insufficient to capture the loss of quality at every word position. 
%This is essential to make sure that system motivated towards reducing \acrshort{ts} is not only triggering searches for the last few positions and the quality of ranking is maintained throughout the query. 
%Figure \ref{fig:line_chart} compares \acrshort{set} with \acrshort{dqn} in terms of the quality of the ranked results returned at every token position. 
%We apply the \acrshort{dqn} agent to filter Instant Searches on unseen test queries for all the datasets. 
%We replay the Inference Algorithm \ref{algo_dqn_agent} that goes over every query $q$ in the test set and emulates Instant Search by providing new tokens to the agent at every time-step $t$. In response, agent picks SEARCH/WAIT action and the result list is updated accordingly. 
%We keep track of the MAP achieved at every time-step $t$ and in the end it is averaged over all the queries. 
%Similar process is repeated for \acrshort{set} which mimics true Instant Search. Figure \ref{fig:line_chart} plots the average MAP(y-axis) at every time-step $t$(x-axis) for both \acrshort{set} and \acrshort{dqn}. As can be observed from these charts, MAP achieved by \acrshort{dqn} is very close to that of \acrshort{set} for all the token positions. This further demonstrates that \acrshort{dqn} doesn't develop position bias towards the end tokens and manages to maintain results quality throughout the query while significantly reducing the overall searches to the underlying system. 

%To better capture the loss of quality in results at every token, we are plotting the average MAP over all the queries at every token position for proposed \acrshort{dqn} model and comparing it with the ideal \acrshort{set} instant search method. 
To further learn more about the proposed DQN model, we have performed detailed analysis of this method. To capture the loss of quality in results at every token, we are plotting the average MAP over all the queries at every token position for the proposed DQN and comparing it with the ideal SET instant search method. 
%We replay the Inference Algorithm \ref{algo_dqn_agent} that goes over every query $q$ in the unseen test set and emulates Instant Search by providing new tokens at every time-step $t$.
We replay the Inference Algorithm \ref{algo_dqn_agent} that goes over queries in the test set and emulates Instant Search by providing new tokens at every time-step $t$.
Based on actions taken by agent, returned results are updated and we keep track of the MAP achieved at every word. Figure \ref{fig:line_chart} plots the average MAP(y-axis) at every time-step $t$(x-axis) for both SET and DQN. Plots show that MAP achieved by DQN is very close to that of SET at all the token positions. This further proves that DQN does not develop position bias towards the end tokens and manages to maintain results quality throughout the query.
\begin{figure}[t]
\centering
    \includegraphics[width=\linewidth]{sayt-len-metrics.jpg}
    \caption{Average MAP achieved by DQN vs SET at every token position. X-axis is token index and Y-axis is MAP averaged over all the queries.}
    \label{fig:line_chart}
\end{figure}
\begin{table}[t]

\scriptsize
\center
\resizebox{\linewidth}
{!}
{
\begin{tabular}{|c|cccccccc|}
\hline
Dataset  & \multicolumn{8}{c|}{Query}                                                                                                                                                                                                                                                                    \\ \hline
MS Marco & labor                          & cost                          & to                              & install                         & tile                           & shower                          &                                 &                                                     \\
         & {\color[HTML]{009901} S,0.03}  & W,-0.01                       & {\color[HTML]{000000} W,0}      & {\color[HTML]{000000} W,0}      & {\color[HTML]{009901} S,0.247} & {\color[HTML]{009901} S,0.25}   & {\color[HTML]{009901} }         &                                                     \\ \hline
MS Marco & what                           & is                            & the                             & purpose                         & of                             & the                             & neutral                         & wire                                                \\
         & W,0                            & W,0                           & {\color[HTML]{000000} W,0}      & {\color[HTML]{000000} W,0}      & W,0                            & {\color[HTML]{000000} W,0}      & {\color[HTML]{009901} S,0.2}    & \multicolumn{1}{l|}{{\color[HTML]{009901} S,0.049}} \\ \hline
INS QA   & What                           & do                            & vest                            & mean                            & in                             & a                               & retirement                      & plan                                                \\
         & W,0                            & W,0                           & {\color[HTML]{009901} S, 0.004} & {\color[HTML]{009901} S, 0.11}  & W,0                            & {\color[HTML]{009901} S, 0.018} & {\color[HTML]{009901} S, 0.208} & {\color[HTML]{009901} S, 0.25}                      \\ \hline
INS QA   & Do                             & home                          & insurance                       & cover                           & a                              & toilet                          & leak                            &                                                     \\
         & W,0                            & W,0                           & {\color[HTML]{009901} S, 0.001} & {\color[HTML]{009901} S, 0.006} & W,0                            & {\color[HTML]{009901} S, 0.01}  & {\color[HTML]{009901} S, 0.155} &                                                     \\ \hline
Wiki IR  & chief                          & justice                       & of                              & new                             & zealand                        &                                 &                                 &                                                     \\
         & {\color[HTML]{009901} S,0.025} & W,0                           & W,0                             & W,0  & {\color[HTML]{009901} S,0.042} &                                 &                                 &                                                     \\ \hline
Wiki IR  & juan                           & carlos                        & i                               & of                              & spain                          &                                 &                                 &                                                     \\
         & {\color[HTML]{009901} S,0.027} & {\color[HTML]{009901} S,0.04} & W,0                             & W,0                             & {\color[HTML]{009901} S,0.188} &                                 &                                 &                                                     \\ \hline
\end{tabular}
}
\caption{Prediction of DQN Network on unseen queries. }

%At every new word, the action taken by the DQN model for the updated query is printed. Here, S is SEARCH and W is WAIT. To further investigate the impact of the action, we are also printing the improvement in MAP caused by triggering the search for the typed query until that token.}
\label{tbl:queries}
\end{table}

%Lastly, to further develop insight into the model beyond just performance metrics, we hand-picked few unseen examples from each dataset and subjectively analysed the actions predicted by the agent. 
Lastly, we hand-picked unseen examples from each dataset and subjectively analysed the actions predicted by the agent. 
Table \ref{tbl:queries} lists couple of queries per dataset and further reports the actions: $W$ for WAIT and $S$ for SEARCH.
%For every new word, we also report the incremental difference in MAP "$\Delta MAP$" observed by including the token into the query and issuing the search. 
For every new word, we also report the incremental difference in MAP $\Delta MAP$ introduced by including the word into the query and issuing the search. 
This allows us to evaluate the quality of actions taken by the agent. Ideally, the agent is expected to pick WAIT action for new words resulting in 0 or negative $\Delta MAP$ and trigger SEARCH for the tokens that improve the MAP for the query. 
%On the contrary, we don't want to skip searches for tokens that can lead to a positive $\Delta MAP$. 

For the MS Marco dataset, besides stopwords, the agent decides to wait for the words \textit{``cost'' }, \textit{``install''} and \textit{``purpose''}. These tokens do not contribute to an improvement in ranking as the reported $\Delta MAP$ is 0. This can be explained by the fact that MS Marco is a large QA dataset with verbose passages. For a simple retriever such as BM25, it is very difficult to retrieve the correct document without more context. The model uses this as a signal to wait for new tokens before triggering a search. 
%Same is true in case of second example where word \textit{"purpose"} appears early on without much context.
%This can be attributed to the fact that MS Marco is a complicated dataset served by a very simple retrieval engine BM25. 
%Often documents in MS Marco talk about actions such as \textit{"install"} without including any explicit mention of the actual term. 
%As BM25 performs a simple term-match, it is incapable of retrieving documents when a query word is absent. 
%This is reflected by the $\Delta MAP$ being 0 for these tokens. 
%In the second example, agent observes a very low IDF token  \textit{"purpose"} early on in the sentence and decides to skip search, as without any extra context it is quite ambiguous. It is important to notice that, agent has learned these behaviors by receiving feedback from the search system during the training.

%For the Insurance QA, we have employed a more sophisticated Semantic Based Matching retriever. 
%This also gets reflected in the actions taken by the agent. 
In the case of InsuranceQA, for the query \textit{``What do vest mean in a retirement plan''} the agent decides to execute the search for the token \textit{``a''}. 
%This is due to the fact that in Insurance jargon, "vest a retirement plan" is a very common phrase. 
In Insurance jargon, ``vest a retirement plan'' is a very common phrase which also explains a positive $\Delta MAP$ introduced by token \textit{``a''} when searched using a sophisticated semantic model such as Universal Sentence Encoder. 
%Positive $\Delta MAP$ for this token highlights that semantic model does not simply treat \textit{"a"} as a stopword and utilizes it to further improve the search quality. Agent picks up this behavior and executes the SEARCH action when it observes \textit{"a"} in this particular context. 
On the contrary, in the second sentence, the same token in a different context is skipped. Also in the insurance jargon \textit{``home''} is a very common term and hence is ignored by the agent early on in the sentence. 

Wiki IR queries are small and usually represent entities such as locations or person names. In the query \textit{``chief justice of new zealand''}, phrase \textit{``chief justice''} often is present as a whole in documents and any improvement in ranking contributed by the phrase is already captured by the rare word \textit{``chief''}. In the second example \textit{``juan carlos i of spain''}, the name \textit{``juan carlos''} itself is unique enough to provide the relevant ranking and does not gain much from the token \textit{``i''}.
%This is a common pattern particular to the Wiki IR dataset queries as observed by the agent during the training. 

==> conclusions.tex <==
In this paper, we study the impact of context and contextual models on citation worthiness. We propose two new formulations for this problem: sentence-pair classification and sentence sequence modeling. We contribute a new benchmark dataset with document-level train/dev/test splits, which enables to incorporate contextual information better. We propose a hierarchical BiLSTM approach for sequence modeling, but we could also consider a transformer-based approach and further improve with a CRF layer. Likewise, we also want to consider some of the newer language models \cite{zaheer2020big,beltagy2020longformer} that handle longer sentences. 

We expect citation worthiness would be an important part of developing writing assistants for scientific documents. We studied the citation worthiness of sentences in scholarly articles in this paper, but we believe these findings are relevant to other domains like news, Wikipedia, and legal documents.

==> discussion.tex <==



==> experiments.tex <==
\label{ssec:datasets}
\begin{comment}

We have evaluated aforementioned approaches on following 3 popular IR datasets:
\begin{itemize}
\item \textbf{MS Marco Passage Ranking}: MS Marco passage ranking\cite{Campos2016MSMA} is a large scale question answering dataset that includes a pool of 8.8 Million passages extracted from 3.2 million documents. For the task of passage re-ranking, dataset further offers more than 1 million queries with their corresponding relevance judgements. Our experiments make sense only when the underlying search engine is able to retrieve relevant documents in top k positions. To ensure that, we have limited the total number of passages by random sampling to 400,000 so that a basic retriever such as BM25 can return relevant documents in top 1000 for a decent number of queries. We have kept 1000 queries with $recall@1000=1$ as  unseen test set. 
\item \textbf{Wiki IR Dataset}: Wiki IR\cite{frej2019wikir} is a recent large-scale standard ad-hoc retrieval dataset. The authors of the dataset have mined Wikipedia documents to automatically extract queries and corresponding relevant documents. For our experiments we are directly utilizing the 59k dataset available on their website. This dataset consists of 59,000 queries with a total document collection of 2.4 million. Similar to MS Marco, we have narrow down the entire universe of documents to 500,000 and reserved 1000 queries with $recall@1000=1$ as  unseen test set. 
\item \textbf{Insurance QA}: The earlier mentioned datasets are more suited for the standard task of Adhoc Retrieval. To further explore the effectiveness of our model in a Question Answer Selection setting, we are experimenting with a  very popular QA dataset known as InsuranceQA\cite{Feng2015ApplyingDL}. Insurance QA is a fairly decently sized QA dataset with a total collection size of 27,413 answers. Dataset also offers a training query set of size 12,889 queries. Inspired by \cite{Tran2018MultihopAN}, this dataset has been adapted to a pure Document Retrieval task. We index all the answers and retrieve top k matched answers for a given question. Insurance QA also offers a test set of 2000 queries. After filtering out queries with $recall@1000=1$, test set is reduced to 821 queries.
\end{itemize}
\end{comment}
We have evaluated aforementioned approaches on the following three popular IR datasets: MS Marco passage ranking\cite{Campos2016MSMA}, Wiki IR\cite{frej2019wikir} and  InsuranceQA\cite{Feng2015ApplyingDL}. For Wiki IR, we are using the 59k version available on authors website. We have followed \cite{Tran2018MultihopAN} to adapt InsuranceQA to a pure Document Retrieval task. Our experiments make sense only when the underlying search engine is able to retrieve relevant documents in top k positions. To ensure that, we have limited the total number of passages by random sampling so that a basic retriever such as BM25 can return relevant documents in top 1000 for a decent number of queries. As a result of the sampling, the total corpus size is reduced to 400,000 and 500,000 for MS Marco and Wiki IR respectively. For InsuranceQA, we use the full set of 27,413 documents. The evaluations set of size 1000 queries is kept unseen during the training for all three datasets.

To showcase the universal applicability of our approach, we conduct experiments using both the term and semantic based matching retrieval systems. For simple term based matching, the very popular BM25\cite{Robertson2009ThePR} algorithm is employed. For semantic retrieval, we use a transformer based pre-trained sentence encoding model known as Universal Sentence Encoder (USE) \cite{cer2018universal} for representing queries and documents with embeddings and further use cosine similarity to rank results.

\begin{comment}\subsection{Retrieval Engines} 
In this section, we cover the details of retrieval engines that have been explored in order to serve the datasets mentioned in the last section. To showcase the universal applicability of our approach, we conduct experiments using both term and semantic based matching retrieval systems. For simple term based matching, very popular BM25\cite{Robertson2009ThePR} algorithm is employed. BM25 ranks documents for a given query based on the relevance score calculated using tf-idf matching between  query and document terms. In our study, BM25 is used in conjunction with traditional adhoc retrieval MS Marco and Wiki IR datasets. Furthermore, in order to support easy replication of results, python's rank-bm25 implementation has been used.

With the recent advent of deep learning, semantic based matching algorithms have gained a lot of popularity. Semantic matching algorithms have been shown to be capable of matching query-document pairs even when they don't share common terms. For our task, we rely on a very recent pre-trained sentence encoding model known as Universal Sentence Encoder (USE) \cite{cer2018universal}. USE is a transformer based model that encodes text into an embedding vector that captures the contextual semantic information present in the input text. USE makes up for limited supervised training data by training on multiple Transfer Learning tasks. For the document retrieval task, USE generates embeddings for query and documents. For a given query, documents are further ranked based on the cosine similarity between the query and document embeddings. In this paper, USE is used with Insurance QA to retrieve relevant answers for the input questions. 
\end{comment}
For \acrshort{sm}, we set a threshold of 0.1.
For the proposed \acrshort{dqn} agent, we trained the model with following settings: future reward $\gamma=0.05$, $\epsilon=1$, $\epsilon_{decay} =0.995$, learning rate $\alpha=0.01$ and $\epsilon_{min}=0.7$. 
Furthermore, weights are learned using Adam optimizer\cite{kingma2014adam} with a batch size of 32.
Reward threshold $R_{th}$ mentioned in reward section for determining the action is set to 0 for MS Marco and Wiki IR and 0.0001 for Insurance QA. 


==> figure.tex <==
\begin{comment}
\begin{figure}
\centering
\begin{tikzpicture}
\node[text height=0.3cm] (y1) {$l_1$};
\node[text height=0.3cm] (y2) [right=of y1] {$l_2$};
\node[text height=0.3cm] (y3) [right=of y2] {$l_3$};
\node[text height=0.3cm] (yn) [right=of y3] {$l_n$};
\node[box,fill=black!10] (h1) [below=0.5 of y1] {$\overleftrightarrow{h_1}$};
\node[box,fill=black!10] (h2) [below=0.5 of y2] {$\overleftrightarrow{h_2}$};
\node[box,fill=black!10] (h3) [below=0.5 of y3] {$\overleftrightarrow{h_3}$};
\node[box,fill=black!10] (hn) [below=0.5 of yn] {$\overleftrightarrow{h_n}$};
\node[text height=0.3cm] (x1) [below=0.5 of h1] {$x_1$};
\node[text height=0.3cm] (x2) [below=0.5 of h2] {$x_2$};
\node[text height=0.3cm] (x3) [below=0.5 of h3] {$x_3$};
\node[text height=0.3cm] (xn) [below=0.5 of hn] {$x_n$};
\node[text height=0.3cm] (bert1) [below=0.5 of x1] {};
\node[text height=0.3cm] (bert2) [below=0.5 of x2] {};
\node[text height=0.3cm] (bert3) [below=0.5 of x3] {};
\node[text height=0.3cm] (bertn) [below=0.5 of xn] {};
\node[text height=0.3cm] (s1) [below=0.5 of bert1] {$s_1$};
\node[text height=0.3cm] (s2) [below=0.5 of bert2] {$s_2$};
\node[text height=0.3cm] (s3) [below=0.5 of bert3] {$s_3$};
\node[text height=0.3cm] (sn) [below=0.5 of bertn] {$s_n$};
\node[text width=2cm] (BiLSTM) [right=0.5cm of hn] {BiLSTM};
\node[text width=2cm] (Input) [right=0.5 of sn] {Sentences};
\node[text width=2cm] (Output) [right=0.5 of yn] {Outputs};
\node[text width=2cm] (BertLayer) [right=0.5 of bertn] {Embedding Layer};
\node[text width=2cm] (Embeddings) [right=0.5 of xn] {Embeddings};
\node[box,minimum width=5.5cm] (bert) [left=0.2 of BertLayer] {Contextual Embedding};
\path (y3) -- node[auto=false]{\ldots} (yn);
\draw[latex'-latex'] (h1) -- node[] {} (h2);
\draw[latex'-latex'] (h2) -- node[] {} (h3);
\path (h3) -- node[auto=false] {\ldots} (hn);
\path (h1) edge [connect] (y1);
\path (h2) edge [connect] (y2);
\path (h3) edge [connect] (y3);
\path (hn) edge [connect] (yn);
\path (x1) edge [connect] (h1);
\path (x2) edge [connect] (h2);
\path (x3) edge [connect] (h3);
\path (xn) edge [connect] (hn);
\path (bert1) edge [connect] (x1);
\path (bert2) edge [connect] (x2);
\path (bert3) edge [connect] (x3);
\path (bertn) edge [connect] (xn);
\path (s1) edge [connect] (bert1);
\path (s2) edge [connect] (bert2);
\path (s3) edge [connect] (bert3);
\path (sn) edge [connect] (bertn);
\path (s3) -- node[auto=false]{\ldots} (sn);
\end{tikzpicture}
\caption{BiLSTM architecture for citation worthiness.}
\label{fig:architecture}
\end{figure}
\end{comment}

==> method.tex <==
\subsection{Problem Statement}
Let $d = \{s_1, s_2, ..., s_n\}$ be a scientific article, where $s_i$ is the $i^{th}$ sentence. The problem of citation worthiness is to assign each sentence $s_i$ one of two possible labels $L = \{l_c, l_n\}$, where $l_c$ denotes that sentence requires a citation and $l_n$ means otherwise. We present three different formulations here to investigate our main research objectives.
% and compare our work with prior research. 

\begin{figure*}[t]
\centering
\includegraphics[width=14cm]{cw_diagram.png}
\caption{The three proposed architectures.}
\label{fig:architectures}
\end{figure*}


\subsection{Sentence Classification}
% \label{sec:sentence}
Our first formulation (Figure \ref{fig:architectures} (a)) approaches citation worthiness as a sentence level classification task similar to prior works of \cite{bonab2018citation,farber2018cite}. Given a sentence $s_i$, we map it to a fixed-size dense vector $x_i$ using contextual embedding models (e.g. BERT \cite{devlin2019bert}). We then feed $x_i$ to a feed-forward layer to obtain the citation worthiness label. We fine-tune this entire architecture by optimizing the weights of the final layer.

\subsection{Sentence-Pair Classification}
\label{sec:sentence-pair}
Our second approach (Figure \ref{fig:architectures} (b)) is to formulate citation worthiness as a sentence-pair classification task, where the pair consists of the given sentence and a sentence-like representation of the context. Namely, for a given sentence $s_i$, we define the context $c_i$ as the concatenation of the previous $s_{i-1}$, $s_i$, and the next sentence $s_{i+1}$: 
\begin{equation}
\label{eq:1}
    c_i = [s_{i-1};s_i;s_{i+1}]
\end{equation}
We then concatenate $s_i$ with $c_i$ separated by the [SEP] token, pass it through the embedding layer to obtain a vector representation $x_i$. This vector is then passed through a feed-forward layer to obtain the class label. This approach is similar to \cite{zeng2020modeling}, where the authors used Glove embeddings \cite{pennington2014glove} to obtain sentence representations, and BiLSTMs for context representations. This formulation has also been used previously for question-answering \cite{devlin2019bert} and passage re-ranking \cite{nogueira2019passage}. In our sentence-pair classification approach, we defined $c_i$ to include only two adjacent sentences, but it could easily include more. However, if we included too many sentences, the context might be too long for most transformer-based models. 

% \label{sec:sentence-sequence}
% \textbf{TODO: Should we add a bit more motivation on why we are considering this model? Reviewers can say that we can use entire context in the sentence pair model. Possible motivation can be that Transformer based models have token length limitation. So it is not easy to include very long sequences of sentences. By modeling this as a sequence of Transformer models, the architecture becomes more scalable to applications where even longer context is needed while keeping the power of transformer models. Feel free to ignore it if you think this makes it more complicated.}
\subsection{Sentence Sequence Modeling}
The third formulation addresses citation worthiness as a sequence labeling task solved using a hierarchical BiLSTM architecture (Figure \ref{fig:architectures} (c)). We first map each sentence $s_i$ and context $c_i$ (eq. \ref{eq:1}) to a fixed-size dense vector $x_i$ using the same approach as in section \ref{sec:sentence-pair}. Thus the given document $d$ is represented as a sequence of vectors $x = \{x_1, x_2, ..., x_n\}$. We then feed these vectors to a BiLSTM model to capture the sequential relations between the sentences. The hidden state of the BiLSTM $h_i$ provides a vector representation for sentence $s_i$ that incorporates information from the surrounding sentences. Thus the sequence modeling approach captures long term dependencies between the sentences without us needing to explicitly encode them as extra features. We then use a feed-forward layer to map the BiLSTM output to the citation worthiness labels. We have also experimented with using only the sentence $s_i$ to construct the vector $x_i$. However, we observed that using the context $c_i$ helped improve the model performance. 

% The variants we consider are based on changing the input embeddings and architecture choices that allow us to incorporate different level of contextual knowledge. 

%We approach this problem as sequence labeling task specifically solved using a hierarchical BiLSTM architecture, which is shown in Figure \ref{fig:architecture}. We first map each sentence $s_i$ to a fixed size dense vector $x_i$ using a contextual embedding layer. Thus the given document $d$ is represented as a sequence of vectors $x = \{x_1, x_2, ..., x_n\}$. We then feed these vectors to a BiLSTM model which captures the sequential relations between the sentences. The hidden state of the BiLSTM $h_i$ is associated with sentence $s_i$. Thus $h_i$ provides a fixed-size representation for sentence $s_i$ while incorporating information from the surrounding sentences. We then apply an affine transformation to map the output of BiLSTM to the citation worthiness labels. 

% \subsection{Contextual vs. Fixed Embeddings}
% We first study the impact of different ways the input sentences can be represented. We compare the performance of contextual embedding models against the state-of-the-art results presented in prior works that use fixed embedding models such as word2vec \cite{mikolov2013distributed} and Glove \cite{pennington2014glove}. Word embeddings are continuous vector representations that are used to initialize words present in a sentence. Fixed word embeddings always produce the same representation irrespective of the context under which a word exists. Contextual  word  embeddings  extend  this  concept to obtain different word representations for the same token based on its context. We fined-tuned three contextual embedding models (BERT \cite{devlin2019bert}, SciBERT \cite{beltagy2019scibert}, and Roberta \cite{liu2019roberta}). Fine-tuning is the process of adding an untrained layer on top of a contextual embedding model and then training the layer weights for a task-specific objective. 
% \subsection{Modeling choices for Additional Context}
% While contextual embeddings enable the model to capture context within the sentence, it alone is not powerful enough to model additional context that is present in the text. This additional context is usually available in the form of surrounding text or the name of the section in which the sentence exists. In this section we will describe the modeling architectures that allow us to capture additional context of different types and sizes.
% \subsubsection{No Context Single Sentence Model}
% This covers models that only use the given sentence text for training and prediction.
% \subsubsection{Limited Context Sentence Pair Model}
% This will cover the method that models neighboring sentences as a sentence pair classification task.
% \subsubsection{Full Context Sequence Model}
% We approach this problem as sequence labeling task specifically solved using a hierarchical BiLSTM architecture, which is shown in Figure \ref{fig:architecture}. We first map each sentence $s_i$ to a fixed size dense vector $x_i$ using a contextual embedding layer. Thus the given document $d$ is represented as a sequence of vectors $x = \{x_1, x_2, ..., x_n\}$. We then feed these vectors to a BiLSTM model which captures the sequential relations between the sentences. The hidden state of the BiLSTM $h_i$ is associated with sentence $s_i$. Thus $h_i$ provides a fixed-size representation for sentence $s_i$ while incorporating information from the surrounding sentences. We then apply an affine transformation to map the output of BiLSTM to the citation worthiness labels.





==> related-work.tex <==
Instant Search has been well studied in the past by the IR community. Various different solutions have been proposed to address the performance and scalability issue towards making this paradigm more easier and practical to employ. A dominant approach considered by many of these studies is based on designing more efficient index data structures that are better suited for this task~\cite{Bast2006TypeLF,Fafalios2011ExploitingAM,Li2012SupportingET}. These data structures are examined together with techniques such as caching ~\cite{Fafalios2012ScalableFA} for their ability to improve search engine query throughput. There has been another thread of research that has studied fuzzy search in conjunction with Instant Search~\cite{ji2009efficient,Li2011EfficientFF,Wang2010InteractiveAF}. Fuzzy search allows the system  to retrieve those records that include words similar to the keywords in the query, even if they do not match exactly. All the mentioned solutions require redesign of the internal search engine mechanics and hence are often complicated to implement. In addition, the final implementation can not be used across different search engine implementations. Our approach mitigates these risks by being agnostic to the underlying search engine.

Recently, reinforcement learning has been successfully applied to an identical problem in the field of Simultaneous Machine Translation (SMT)~\cite{grissom,satija2016simultaneous,Neubig2017LearningTT}. SMT is defined as the task of producing a real-time translation of a sentence while typing. The goal here is to achieve a good trade-off between the quality and delay of the translation. In this paper, we further extend this idea to learn query term importance and use it to selectively trigger Instant Search. 

==> related.tex <==
Citation worthiness is very closely related to citation recommendation, where the goal is to recommend a reference for a sentence in a scientific article. Many of these studies have proposed techniques that incorporate local context into the ranking process. \cite{strohman2007recommending} linearly combine text and citation-based features to generate scores for the final ranking task. \cite{he2010context} designed a context-aware non-parametric probabilistic model to measure the relevance between a citation and a document. More recently, neural networks have been explored by \cite{huang2015neural, ebesu2017neural} to select and rank citations for a given article. \cite{cai2018three, yang2018lstm, cai2018generative} further extended the research area by combining penalization into the recommendation process.  

Citation analysis, another closely related research domain, aims to predict the sentiment and purpose of a citation. \cite{athar2012context} used the context to predict the sentiment of a citation and explored the effects of context size on the final performance. \cite{abu2013purpose} presented a sequence labeling model that identifies the context and classifies the polarity. \cite{athar2011sentiment} explored the effectiveness of structured-based features for this task. While most of the current research trains separate models for the sentiment and purpose identification tasks, \cite{yousif2019multi} proposed a multi-task learning setup that jointly learns the objectives for these two tasks. 

Recognizing and understanding the author's motivation behind a citation has also been well studied by NLP researchers, commonly referred to as citation function classification. \cite{teufel2006automatic} proposed a new annotation scheme and explored supervised learning to solve this task. \cite{li2013towards} expanded on this annotation scheme by including more functions and implementing a Maximum Entropy-based system to classify citation functions automatically. Recently, \cite{hernandez2017citation} presented a new annotation scheme that produces a more granular set of categories for this classification task.

% Citations within the scientific literature have been well studied in the context of problems that are closely related to the task of citation worthiness. One such research area involves applying machine learning models towards the goal of recommending citations for a given scientific article. Many of these studies have proposed techniques that incorporate local context into the ranking process.
% \cite{strohman2007recommending} linearly combines text and citation based features in order to generate scores for the final ranking task. \cite{he2010context} designed a context-aware non-parametric probabilistic model to measure the relevance between a citation and a document. Very recently neural networks have been explored by \cite{huang2015neural, ebesu2017neural} to select and rank citations for a given article. \cite{cai2018three, yang2018lstm, cai2018generative} further extended the research area by combining penalization into the recommendation process.  

% Citation Analysis is a research area that studies and predicts the sentiment and purpose of a citation with respect to the citation context. \cite{athar2012context} applies the context towards predicting the sentiment of a citation and explores the effects of context size on the final performance. \cite{abu2013purpose} presented a sequence labeling model that identifies the context and classifies polarity based on it. \cite{athar2011sentiment} explores in detail the effectiveness of structured based features for this task. While most of the current research trains separate models for the sentiment and purpose identification tasks, \cite{yousif2019multi} proposed a multi-task learning setup that jointly learns the objectives for these two tasks. 

% Recognizing and understanding the author's motivation behind a citation has also been well studied by researchers from different fields. This task is commonly referred as citation function classification. \cite{teufel2006automatic} proposed a new annotation scheme and further explored supervised learning to solve the task. Later \cite{li2013towards} expanded on this annotation scheme by including more functions and implemented a Maximum Entropy-based system to automatically classify citation functions. Recently \cite{hernandez2017citation} presented a new annotation scheme that manages to produce more granular set of categories for the classification task.
